Quantum law of large numbers for Banach spaces

We consider random operators $\Omega \to \mathcal{L}(\ell_p, \ell_p)$ for some $1 \leqslant p < \infty$. The law of large numbers is known in the case $p=2$ in the form of usual law of large numbers. Instead of sum of i.i.d. variables there may be considered the composition of random semigroups $e^{A_i t/n}$. We obtain the law of large numbers for the case $p \leqslant 2$.

==> listmain.tex <==
\newcommand{\setenumi}{
    \topsep=0mm
    \partopsep=0mm
    \parsep=0mm
    \itemsep=0mm
    \leftmargin=0pt
    \listparindent=7mm
    \itemindent=3mm
    \labelsep=2mm
    \labelwidth=-5mm
    \usecounter{enumi}
    }



% \newcommand{\setitemi}{
%     \topsep=0mm
%     \partopsep=0mm
%     \parsep=0mm
%     \itemsep=0mm
%     \leftmargin=\leftmargini
%     \listparindent=0mm
%     \itemindent=0mm
%     \labelsep=2mm
%     \labelwidth=3mm
%     }    

\newenvironment{remarkenumi}
    {\begin{list}{\labelenumi}{\setenumi}}
    {\end{list}}

% \renewenvironment{itemize}
%     {\begin{list}{$\bullet$}{\setitemi}}
%     {\end{list}}

\renewcommand{\theenumi}{\alph{enumi}}
\renewcommand{\labelenumi}{(\alph{enumi})}

